Adiabatic replay for continual learning

Conventional replay-based approaches to continual learning (CL) require, for each learning phase with new data, the replay of samples representing all of the previously learned knowledge in order to avoid catastrophic forgetting. Since the amount of learned knowledge grows over time in CL problems, generative replay spends an increasing amount of time just re-learning what is already known. In this proof-of-concept study, we propose a replay-based CL strategy that we term adiabatic replay (AR), which derives its efficiency from the (reasonable) assumption that each new learning phase is adiabatic, i.e., represents only a small addition to existing knowledge. Each new learning phase triggers a sampling process that selectively replays, from the body of existing knowledge, just such samples that are similar to the new data, in contrast to replaying all of it. Complete replay is not required since AR represents the data distribution by GMMs, which are capable of selectively updating their internal representation only where data statistics have changed. As long as additions are adiabatic, the amount of to-be-replayed samples need not to depend on the amount of previously acquired knowledge at all. We verify experimentally that AR is superior to state-of-the-art deep generative replay using VAEs.

==> tables_outsourced.tex <==
%%%%%%%%%%%% MNIST %%%%%%%%%%%
\section{Full results: MNIST} 
%
\begin{table}[h!]
%\setlength{\arrayrulewidth}{0.1mm}
%\renewcommand{\arraystretch}{1.}
%\setlength{\tabcolsep}{6pt}
\small
\centering
\begin{tabular}{c c | c | c | c}
    \hline
    \multicolumn{5}{c}{\textbf{MNIST}} \\
	\hline
	\multicolumn{2}{c}{}                        				& \multicolumn{3}{|c}{\textbf{test acc./std. (\%) for $D_i$ after $T_i$}} \\	
	\textbf{task} & \textbf{test on}            				& \textbf{AR} & \textbf{DGR(c.)} & \textbf{DGR(b.)} \\                               
	\hline\hline
	\textit{base}                	 							& $T_{ALL}$ & $89.8$ $\pm 0.6$ & \multicolumn{2}{c}{$97.7$ $\pm 0.3$} 	\\
	\hline\hline                                 				% 7-1A
	                                            				& $T_{ALL}$ 		& 78.0 $\pm0.4$ 	& 74.9 $\pm2.5$ 	& 90.3 $\pm0.9$ 		\\
	                                            				& $T_1$     		& 79.9 $\pm1.7$ 	& 67.1 $\pm2.9$ 	& 90.7 $\pm1.7$ 		\\
	\multirow{2}{*}{\textbf{D7-$1^3$a}}   					    & $T_2$     		& 64.7 $\pm8.1$ 	& 86.3 $\pm3.4$ 	& 82.3 $\pm2.7$		\\
	                                            				& $T_3$     		& 67.8 $\pm0.8$ 	& 93.9 $\pm2.1$ 	& 89.2 $\pm3.2$ 		\\
	                                            				& $T_4$     		& 80.2 $\pm5.9$ 	& 98.2 $\pm0.6$ 	& 97.3 $\pm0.4$ 		\\
	\hline                                 
	                                            				% 7-1B 
	                                            	           	& $T_{ALL}$		& 83.1 $\pm0.4$ 	& 82.5 $\pm0.7$	& 94.9 $\pm0.3$ 		\\
	                                            				& $T_1$     		& 82.8 $\pm1.2$ 	& 75.2 $\pm0.9$	& 93.8 $\pm0.6$ 		\\
	\multirow{2}{*}{\textbf{D7-$1^3$b}}   					    & $T_2$     		& 84.6 $\pm2.9$ 	& 97.9 $\pm0.7$	& 97.3 $\pm0.6$		\\
	                                            				& $T_3$     		& 94.2 $\pm4.1$ 	& 99.1 $\pm0.2$	& 98.1 $\pm0.4$ 		\\
	                                            				& $T_4$     		& 68.6 $\pm4.4$ 	& 98.2 $\pm0.7$ 	& 96.6 $\pm1.3$ 		\\
	\hline\hline                                 
	                                            				% 6-1A
					                                        	& $T_{ALL}$		& 76.1 $\pm1.7$ 	& 66.2 $\pm3.5$ 	& 88.3 $\pm1.2$      \\
					                                         	& $T_1$     		& 79.7 $\pm2.7$ 	& 49.4 $\pm6.2$ 	& 87.1 $\pm1.4$      \\
					                                         	& $T_2$     		& 83.5 $\pm4.1$ 	& 90.9 $\pm2.6$ 	& 91.4 $\pm2.9$      \\
	\multirow{2}{*}{\textbf{D6-$1^4$a}}						      & $T_3$			& 62.8 $\pm5.9$	& 82.7 $\pm3.5$ 	& 82.6 $\pm1.6$      \\
					                                        	& $T_4$     		& 60.7 $\pm6.1$ 	& 93.8 $\pm0.6$ 	& 88.9 $\pm1.9$      \\
					                                        	& $T_5$     		& 78.5 $\pm1.7$ 	& 98.7 $\pm0.4$ 	& 97.5 $\pm0.4$      \\
	\hline                                 
	                                            				% 6-1B
					                                         	& $T_{ALL}$		& 79.9 $\pm0.8$ 	& 70.2 $\pm0.3$ 	& 90.7 $\pm0.6$      \\
					                                      	& $T_1$     		& 80.3 $\pm1.1$ 	& 51.2 $\pm0.8$ 	& 86.7 $\pm0.9$      \\
					                                      	& $T_2$     		& 81.9 $\pm1.6$ 	& 95.6 $\pm1.2$ 	& 95.3 $\pm1.9$      \\
	\multirow{2}{*}{\textbf{D6-$1^4$b}}						& $T_3$     		& 96.6 $\pm2.1$	& 98.8 $\pm0.2$ 	& 97.9 $\pm0.7$      \\
					                                      	& $T_4$     		& 71.9 $\pm8.2$ 	& 93.9 $\pm2.9$ 	& 92.9 $\pm1.0$      \\
					                                       	& $T_5$     		& 72.5 $\pm2.9$ 	& 99.1 $\pm0.4$ 	& 98.7 $\pm0.4$      \\
	\hline\hline                                        
															% 5-1A
					                                     		& $T_{ALL}$		& 73.9 $\pm0.6$ 	& 62.5 $\pm2.2$ 	& 83.3 $\pm3.4$      \\
					                                  		& $T_2$     		& 75.2 $\pm3.2$ 	& 40.3 $\pm3.4$ 	& 77.8 $\pm6.1$      \\
					                                         	& $T_3$     		& 64.2 $\pm4.5$ 	& 60.2 $\pm2.0$ 	& 79.3 $\pm3.9$      \\
	\multirow{2}{*}{\textbf{D5-$1^5$a}}						& $T_4$     		& 84.6 $\pm4.8$	& 90.6 $\pm1.6$ 	& 92.7 $\pm1.8$      \\
					                                         	& $T_5$     		& 64.8 $\pm3.2$ 	& 84.9 $\pm2.2$ 	& 83.7 $\pm1.7$      \\
					                                        	& $T_6$     		& 59.9 $\pm4.4$ 	& 93.9 $\pm1.3$ 	& 91.5 $\pm1.1$      \\
					                                        	& $T_7$     		& 81.4 $\pm1.5$ 	& 98.6 $\pm0.2$ 	& 97.9 $\pm0.5$      \\
	\hline                          
															% 5-1B       
					                                         	& $T_{ALL}$		& 75.5 $\pm0.4$ 	& 70.0 $\pm3.1$ 	& 89.7 $\pm0.5$      \\
					                                        	& $T_2$     		& 72.1 $\pm3.2$ 	& 42.9 $\pm5.3$ 	& 83.5 $\pm1.6$      \\
					                                         	& $T_3$     		& 82.9 $\pm7.5$ 	& 88.9 $\pm5.9$ 	& 93.6 $\pm0.9$      \\
	\multirow{2}{*}{\textbf{D5-$1^5$b}}						& $T_4$     		& 93.2 $\pm4.3$	& 98.1 $\pm0.7$ 	& 96.9 $\pm0.5$      \\
					                                         	& $T_5$     		& 69.4 $\pm10.6$	& 93.1 $\pm0.3$ 	& 92.6 $\pm1.6$      \\
					                                        	& $T_6$     		& 69.3 $\pm2.4$ 	& 97.9 $\pm0.4$ 	& 96.7 $\pm0.7$      \\
					                                         	& $T_7$     		& 78.1 $\pm1.9$ 	& 99.5 $\pm0.1$ 	& 97.5 $\pm0.8$      \\

\end{tabular}
\caption{MNIST: Shows experimental results for AR and DGR (balanced and constant-time training scenario). Lists the baseline performance on all dataset classes $T_{ALL}$ for comparison, as well as the evaluation metrics for $T_i$, and $T_{ALL}$ after completion of all sub-tasks ($i=[4,5,6]$). Details about the CL-problems can be found in \cref{tab:slts}). All metrics are calculated after completion of each sub-task and represent the resulting values of the trained model tested on the evaluation data corresponding to the sub-task; metrics are averaged over all experimental runs.
\label{tab:expres_long_mnist}
}
\end{table}
%
\newpage
%%%%%%%%%%%% FMNIST %%%%%%%%%%%
\section{Full results: FashionMNIST}
%
\begin{table}[h!]
%\setlength{\arrayrulewidth}{0.1mm}
%\renewcommand{\arraystretch}{1.}
%\setlength{\tabcolsep}{6pt}
\small
\centering
\begin{tabular}{c c | c | c | c}
    \hline
    \multicolumn{5}{c}{\textbf{FashionMNIST}} \\
	\hline
	\multicolumn{2}{c}{}                        & \multicolumn{3}{|c}{\textbf{test acc./std. (\%) for $D_i$ after $T_i$}} \\
	\textbf{task} & \textbf{test on}            & \textbf{AR} & \textbf{DGR(c.)} & \textbf{DGR(b.)} \\                   
	\hline\hline
	\textit{base}                	 			  & $T_{ALL}$ & $74.1$ $\pm 0.8$ & \multicolumn{2}{c}{$88.6$ $\pm 0.2$} \\
	\hline\hline                               	
	                                            % 7-1A
	                                            & $T_{ALL}$ & 70.3 $\pm1.2$ & 68.9 $\pm1.9$ & 79.9 $\pm1.2$      \\
	                                            & $T_1$     & 64.0 $\pm2.4$ & 59.9 $\pm2.9$ & 76.7 $\pm1.4$      \\
	\multirow{2}{*}{\textbf{D7-$1^3$a}}         & $T_2$     & 73.4 $\pm3.8$ & 72.9 $\pm5.4$ & 69.9 $\pm4.2$      \\
	                                            & $T_3$     & 88.7 $\pm1.2$ & 97.6 $\pm1.0$ & 94.7 $\pm0.4$      \\
	                                            & $T_4$     & 92.1 $\pm0.1$ & 99.2 $\pm0.5$ & 98.6 $\pm0.5$      \\
	\hline                                 
	                                            % 7-1B
	                                            & $T_{ALL}$ & 69.3 $\pm0.3$ & 65.8 $\pm0.7$ & 75.1 $\pm2.8$      \\
	                                            & $T_1$     & 66.0 $\pm2.4$ & 56.0 $\pm1.7$ & 73.1 $\pm4.4$      \\
	\multirow{2}{*}{\textbf{D7-$1^3$b}}         & $T_2$     & 73.1 $\pm1.2$ & 70.4 $\pm5.9$ & 48.6 $\pm1.9$      \\
	                                            & $T_3$     & 82.0 $\pm0.4$ & 97.1 $\pm0.3$ & 96.1 $\pm0.3$      \\
	                                            & $T_4$     & 76.2 $\pm5.5$ & 97.9 $\pm0.6$ & 94.9 $\pm4.7$      \\
	\hline\hline                                 
	                                            % 6-1A
	                                            & $T_{ALL}$ & 67.6 $\pm0.7$ & 65.7 $\pm1.7$ & 76.9 $\pm1.2$      \\
	                                            & $T_1$     & 64.5 $\pm2.8$ & 61.6 $\pm5.1$ & 82.3 $\pm0.4$      \\
	                                            & $T_2$     & 52.8 $\pm7.3$ & 23.1 $\pm20.8$ & 6.2 $\pm8.7$      \\
	\multirow{2}{*}{\textbf{D6-$1^4$a}}         & $T_3$     & 60.2 $\pm4.4$ & 67.7 $\pm11.5$ & 75.6 $\pm4.2$     \\
	                                            & $T_4$     & 79.3 $\pm4.1$ & 96.9 $\pm0.7$ & 94.1 $\pm0.5$      \\ 
	                                            & $T_5$     & 91.9 $\pm3.6$ & 99.6 $\pm0.3$ & 98.8 $\pm0.6$      \\
	\hline                                 
	                                            % 6-1B
	                                            & $T_{ALL}$ & 69.9 $\pm0.7$ & 59.2 $\pm1.0$ & 75.6 $\pm1.3$      \\
	                                            & $T_1$     & 66.1 $\pm4.1$ & 42.4 $\pm2.6$ & 73.5 $\pm1.4$      \\
	                                            & $T_2$     & 53.5 $\pm2.9$ & 57.9 $\pm8.5$ & 48.9 $\pm13.5$     \\
	\multirow{2}{*}{\textbf{D6-$1^4$b}}         & $T_3$     & 84.2 $\pm3.6$ & 92.8 $\pm1.9$ & 93.6 $\pm1.0$      \\
	                                            & $T_4$     & 78.8 $\pm12.4$ & 88.9 $\pm1.0$ & 75.9 $\pm4.9$     \\
	                                            & $T_5$     & 80.9 $\pm1.7$ & 98.0 $\pm1.2$ & 97.2 $\pm0.3$      \\

	\hline\hline                                      
	                                            % 5-1A
	                                            & $T_{ALL}$ & 68.6 $\pm0.7$ & 63.5 $\pm0.8$ & 77.3 $\pm1.4$     \\
	                                            & $T_1$     & 72.3 $\pm2.8$ & 53.1 $\pm4.3$ & 81.7 $\pm2.8$     \\
	                                            & $T_2$     & 41.9 $\pm6.9$ & 44.3 $\pm4.3$ & 74.3 $\pm4.5$     \\
	\multirow{2}{*}{\textbf{D5-$1^5$a}}         & $T_3$     & 44.1 $\pm8.6$ & 52.7 $\pm17.4$ & 17.3 $\pm13.3$   \\
	                                            & $T_4$     & 60.8 $\pm3.9$ & 76.0 $\pm7.3$ & 77.8 $\pm3.1$     \\
	                                            & $T_5$     & 84.3 $\pm3.5$ & 97.1 $\pm0.4$ & 96.1 $\pm0.6$     \\
	                                            & $T_6$     & 95.6 $\pm1.5$ & 99.1 $\pm0.7$ & 99.0 $\pm0.3$     \\
	\hline                                 
	                                            % 5-1B
	                                            & $T_{ALL}$ & 66.9 $\pm0.2$ & 55.7 $\pm5.5$ & 72.0 $\pm0.9$     \\
	                                            & $T_1$     & 73.4 $\pm1.6$ & 43.7 $\pm7.9$ & 73.5 $\pm2.4$     \\
	                                            & $T_2$     & 47.9 $\pm4.2$ & 43.4 $\pm11.8$ & 59.4 $\pm14.2$   \\
	\multirow{2}{*}{\textbf{D5-$1^5$b}}         & $T_3$     & 80.3 $\pm3.9$ & 93.6 $\pm1.0$ & 94.6 $\pm1.2$     \\
	                                            & $T_4$     & 19.3 $\pm2.9$ & 30.2 $\pm2.4$ & 31.4 $\pm12.6$    \\
	                                            & $T_5$     & 74.2 $\pm5.2$ & 72.6 $\pm1.8$ & 71.6 $\pm2.3$     \\
	                                            & $T_6$     & 84.5 $\pm2.1$ & 98.2 $\pm0.6$ & 95.5 $\pm4.6$     \\

\end{tabular}
\caption{FashionMNIST: Shows experimental results for AR and DGR (balanced and constant-time training scenario). Lists the baseline performance on all dataset classes $T_{ALL}$ for comparison, as well as the evaluation metrics for $T_i$, and $T_{ALL}$ after completion of all sub-tasks ($i=[4,5,6]$). Details about the CL-problems can be found in \cref{tab:slts}). All metrics are calculated after completion of each sub-task and represent the resulting values of the trained model tested on the evaluation data corresponding to the sub-task; metrics are averaged over all experimental runs.
\label{tab:expres_long_fmnist}
}
\end{table}
%

%%%%%%%%%%%% EMNIST %%%%%%%%%%%
\newpage
%%%%%%%%%%%% EMNIST %%%%%%%%%%%
\section{Full results: EMNIST}
%
\begin{table}[h!]
%\setlength{\arrayrulewidth}{0.1mm}
%\renewcommand{\arraystretch}{1.}
%\setlength{\tabcolsep}{6pt}
\small
\centering
\begin{tabular}{c c | c | c | c}
    \hline
    \multicolumn{5}{c}{\textbf{EMNIST}} \\
	\hline
	\multicolumn{2}{c}{}                        & \multicolumn{3}{|c}{\textbf{test acc./std. (\%) for $D_i$ after $T_i$}} \\
	\textbf{task} & \textbf{test on}            & \textbf{AR} & \textbf{DGR(c.)} & \textbf{DGR(b.)} \\                                  
	\hline\hline
	\textit{base}                	 			  & $T_{ALL}$ & $44.1$ $\pm 3.3$ & \multicolumn{2}{c}{$84.6$ $\pm 0.1$}   \\
	\hline                               	
	                                            % 20-1A
	                                            & $T_{ALL}$ & 32.6 $\pm1.1$ 	& 12.7 $\pm1.0$ 		& 50.6 $\pm20.9$     \\
	                                            & $T_1$     & 61.9 $\pm3.6$ 	& 9.5 $\pm2.3$ 		& 70.1 $\pm5.9$     \\
	                                            & $T_2$     & 58.4 $\pm3.5$ 	& 57.3 $\pm7.1$ 		& 38.1 $\pm29.3$     \\
	\multirow{2}{*}{\textbf{D20-$1^5$a}}        & $T_3$     & 25.3 $\pm9.5$ 	& 65.3 $\pm6.9$ 		& 36.9 $\pm45.5$    \\
	                                            & $T_4$     & 73.6 $\pm1.7$ 	& 91.3 $\pm2.2$ 		& 87.5 $\pm1.6$     \\
	                                            & $T_5$     & 47.1 $\pm6.2$ 	& 94.1 $\pm1.0$ 		& 92.7 $\pm5.3$     \\
	                                            & $T_6$     & 37.8 $\pm2.9$ 	& 99.2 $\pm0.8$ 		& 94.9 $\pm0.9$     \\
	\hline                                 
	                                            % 20-1B
	                                            & $T_{ALL}$ & 31.2 $\pm0.5$ 	& 14.6 $\pm1.3$ 		& 36.3 $\pm1.3$     \\
	                                            & $T_1$     & 62.7 $\pm4.5$ 	& 13.9 $\pm1.9$ 		& 69.8 $\pm4.1$     \\
	                                            & $T_2$     & 33.7 $\pm7.5$ 	& 46.6 $\pm26.1$ 	& 15.5 $\pm26.9$    \\
	\multirow{2}{*}{\textbf{D20-$1^5$b}}        & $T_3$     & 31.5 $\pm0.8$ 	& 74.8 $\pm13.6$ 	& 24.8 $\pm33.9$     \\
	                                            & $T_4$     & 63.5 $\pm3.1$ 	& 92.2 $\pm2.1$ 		& 83.3 $\pm5.6$    \\
	                                            & $T_5$     & 59.5 $\pm6.2$ 	& 97.0 $\pm0.7$ 		& 92.9 $\pm1.3$     \\
	                                            & $T_6$     & 39.8 $\pm8.5$ 	& 99.4 $\pm0.3$ 		& 95.2 $\pm1.7$     \\

\end{tabular}
\caption{EMNIST: Shows experimental results for AR and DGR (balanced and constant-time training scenario). Lists the baseline performance on all dataset classes $T_{ALL}$ for comparison, as well as the evaluation metrics for $T_i$, and $T_{ALL}$ after completion of all sub-tasks ($i=6$). Details about the CL-problems can be found in \cref{tab:slts}). All metrics are calculated after completion of each sub-task and represent the resulting values of the trained model tested on the evaluation data corresponding to the sub-task; metrics are averaged over all experimental runs.
\label{tab:expres_long_EMNIST}
}
\end{table}
%
